A Fully Homomorphic Encryption Scheme for Real-Time Safe Control

Fully Homomorphic Encryption (FHE) has made it possible to perform addition and multiplication operations on encrypted data. Using FHE in control thus has the advantage that control effort for a plant can be calculated remotely without ever decrypting the exchanged information. FHE in its current form is however not practically applicable for real-time control as its computational load is very high compared to traditional encryption methods. In this paper a reformulation of the Gentry FHE scheme is proposed and applied on an FPGA to solve this problem. It is shown that the resulting FHE scheme can be implemented for real-time stabilization of an inverted double pendulum using discrete time control.

==> Sections/fpga_OLD.tex <==
\noindent In this section it is shown that the reformulation of the FHE scheme using the reduced cipher, as presented in Section \ref{sec:fpga}, is well suited for implementation on an FPGA. Due to the unique hardware structure of an FPGA it can greatly benefit from the reduced computational complexity achieved by using the reduced cipher in FHE. An FPGA is an integrated circuit with hardware components that can be reconfigured to create logic circuits. As such, an FPGA can be configured to act as a conventional CPU or APU or it can be configured as a standalone chip or hardware accelerator with a dedicated design. In this work we will configure the FPGA as a standalone chip. As such the implementation does not have a software layer which allows for efficient implementation of the FHE scheme.

\subsection{Hardware Resources of an FPGA}\label{ssec:fpga_hard}
\noindent An FPGA contains generic logic cells and memory components of differing sizes and configurability. The most common type of logic cell is called Adaptive Logic Modules (ALM), these can be configured to perform any operation. Though ALM's can be configured to perform multiplication, this would be very inefficient and so FPGA's are generally equipped with Digital Signal Processing (DSP) slices which are specifically made to perform multiplication. Unfortunately, due to the die space requirements, there are fewer available. To illustrate, on any particular FPGA, ALM's are usually available in the order of tens of thousands, whereas there are usually only DSP's available in the order of tens. If a design's speed relies on multiplication, the limited amount of available DSP-slices could bottle-neck the computational speed.
%\noindent An FPGA contains generic logic cells which include a lookup table (LUT), some full-adders, flip-flops and multiplexers. These generic units are called Adaptive Logic Modules (ALM). A LUT serves to encode a given input. The full-adders are optional and can perform addition with the output from the LUT and some outside source. The multiplexers determine whether the full-adders are used or not. The flip-flops serve to capture the resulting logic on the rising edge of the clock. ALM's can be efficiently configured to perform a wide range of logical operations. ALM's are efficient in terms of die-space and therefore many thousands to tens of thousands of them can be fit on a single FPGA. Addition is possible, however multiplication cannot be implemented effectively using ALM's and is not recommended. Hence, FPGA's are generally equipped with Digital Signal Processing (DSP) slices. These units require more die-space, and so fewer are available (in the order of tens to hundreds).

%\subsection{Computational Capabilities of an FPGA}\label{ssec:fpga_comp}
%\noindent The hardware resources of an FPGA can be configured freely, either to work as a CPU or APU for general purpose, or as standalone chip to perform a dedicated task. By using the FPGA as a standalone chip, many of the computational bottlenecks of conventional CPUs or APUs can be taken away, at the cost of loosing flexibility. For example, a conventional CPU requires software to drive the hardware, which creates overhead; or when using a GPU for parallel computations, it has to be configured by a CPU and as such its operation is bottle-necked by the speed of communication between GPU and CPU.

%-types of operations.
%The computational capabilities of an FPGA when configured as a standalone chip is dependent mostly on the number and type of operations performed for the algorithm which it implements. Therefore, in the following a distinction will be made between different types of operations, namely additions, multiplications, and bit-operations, each of which will be discussed in more detail below.

%-how can hardware resources be used for these operations.
%Firstly, on an FPGA,  addition can be performed using DSP-slices or using ALM's. However, using DSP's only would be wasteful, given that the amount of DSP's on an FPGA is usually more limited. Alternatively, using ALM's is less direct (logic circuits have to be constructed with ALM's), but is preferable given that they are relatively abundant.

%Secondly, multiplication can be performed only by using DSP-slices. In theory ALMs could also be used for multiplication, however this would be incredibly space-inefficient (in terms of die space). DSP slices are more compact, but they are still comparitively scarce, limiting how fast multiplication can be performed on an FPGA.

%Lastly, bit-operations is a class of operations that can only be performed bit-wise, which include bit-shifts, bit-masks, etc. These operations can be used to replace specific multiplication operations. A bit-shift can be used for multiplications with powers of $2$ and a bit-mask for multiplications with booleans. On an FPGA bit-operations can be performed in the same clock-tick as an addition or multiplication without using any additional resources. Bit-operations are therefore the preferred operation on an FPGA.
\subsection{Using the Reduced Cipher on an FPGA}\label{ssec:fpga_reduced}
\noindent The reduced cipher implementation as presented in Section \ref{sec:fpga} reduces the computational load of the scheme on any platform, however one aspect is particularly beneficial to FPGA design.\\
As shown in Table \ref{tab:hom_oper}, the total number of operations is reduced by an order of magnitude when using the reduced cipher. More importantly however, is that all multiplication operations are replaced by bit-operations and additions. This improvement is specifically useful for implementation on an FPGA. As discussed in Section \ref{ssec:fpga_hard}, reliance on multiplication operations could limit the computational speed of an FPGA. Therefore, by replacing all multiplications with bit-operations, utilisation can be shifted from DSP-slices to ALM's which are abundant.\\
These improvements of the FHE scheme, achieved by using the reduced cipher, combined with the fit-for-purpose hardware of the FPGA, makes it possible to perform encryption, homomorphic operations, and decryption with only a small delay. This allows us to implement encrypted control in real-time with a high update rate. In section \ref{sec:results} it will be shown how a double inverted pendulum can be stabilized using the novel reduced cipher implementation of the proposed FHE scheme. 

==> Sections/introduction_OLD.tex <==
%Why do we look at encryption in the context of safe control
Cryptography has allowed for the development of control-systems, such as hydroelectric dams or energy grids at a regional or larger level, that can be securely monitored and controlled over long distances. Such spatially distributed systems require a connection, either wired or wireless, between plant and controller and hierarchically between controllers. Due to the scale of these systems it is infeasible to fully secure these communication channels from intrusion. Therefore, encryption might be the only way to secure communications in such case.

%Current industry standard & Problems
Currently, industrial control systems are secured at different levels by means of end-to-end encryption, utilising a mix of symmetric-key and public-key encryption schemes \citep{AES,RSA,EncInCrtl}. These methods are successful in securing low rate communication within a large scale control system. However, they are not applicable in the context of high sampling frequency feedback-control, as these schemes require multiple encryption and decryption steps. In particular, sensor data has to be encrypted at the sensor level, transmitted to the controller and then decrypted there to calculate control effort. The latter has to be encrypted by the controller, transmitted to the actuator and then finally decrypted by the actuator before being applied. The time overhead required by these operation introduces delays in the feedback loop that will reduce the stability margin, and possibly de-stabilize the plant. Furthermore the use of decrypted data at the controller level means that these methods do not provide security in case the controller itself is compromised.

%Sensor data and control effort can be encrypted and exchanged. When data arrives at the controller or plant, it has to be decrypted for use. An attacker with access to the communication line will be unable to tamper with the data. However if the attacker gets access to the controller, they could sabotage still the system.

%The idea of homomorphic encryption as a solution to these problems, with refs to types of encryption schemes (general)

A solution to this problem is found in encryption schemes with homomorphic properties, for which operations on encrypted data exist that are equivalent to multiplication and/or addition. The first encryption scheme that had such homomorphic properties was the now ubiquitous RSA encryption scheme \citep{RSA}. Within a year of publication, the idea of Homomorphic Encryption (HME) was introduced \citep{Rivest}. Implementing controllers utilising HME would allow calculating control action without decryption at the controller, thus securing a control system even in case the controller is breached. Furthermore, it will bring the number of encryption and decryption steps down from four, to only two, simplifying the control loop.
%Furthermore, it will bring the number of encryption and decryption steps down from four, to only two, thus easing the risk of de-stabilizing the plant.

HME schemes that followed were schemes such as the El Gamal scheme \citep{ElGamal} and the Paillier scheme \citep{Paillier}, which both derive security from difficulty of computing discrete logarithms over finite fields. These schemes are Partially Homomorphic Encryption (PHE) schemes, which means that they do not support the full range of multiplication and addition of encrypted numbers. The Paillier scheme \citep{Paillier}, for example, only allows for addition of ciphers and the multiplication of a cipher by an unencrypted number.% For encrypted control this means these schemes are limited to only very simple direct feedback controllers.%...**I guess they could only do scalar feedback control? And could they do multiple consecutive multiplications on fractional data?** %These schemes are all similar in that they utilise prime based mathematical problems to encrypt numbers.

More recently lattice-based HME schemes have been introduced by \cite{Gentry2009}, followed by many advances \citep{gentry2013,Cheon2015}.%These schemes would be followed up by lattice based encryption schemes 
%**Add examples of schemes *** \citep{gentry2013}. 
These encryption schemes are Fully Homomorphic Encryption (FHE) schemes, meaning they support both addition and multiplication of encrypted numbers. For encrypted control this means these schemes potentially allow for implementation of a broad range of feedback control. However, the high computational complexity of these lattice based schemes prevents these schemes from being used in real-time on conventional hardware.

%The first control systems utilising HME as proposed by \citep{RTS_HME_FPGA} would utilise combinations of the RSA \citep{RSA}, El Gamal \citep{ElGamal} and the Paillier \citep{Paillier} encryption schemes. All these schemes are Partially Homomorphic Encryption schemes. This means that they only support only a multiplication or addition of encrypted numbers. As a result, to perform control scheme as proposed by \cite{RTS_HME_FPGA} has to leave the state space matrices unencryped. The scheme as proposed by \citep{HME_networked_control}, ....

%Applications of HME for control, their advantages and problems.
Some attempts have been made to use PHE schemes for control. \cite{HME_networked_control} were the first to propose a HME control scheme using the PHE scheme from \cite{ElGamal} combined with the RSA scheme. This control scheme requires the controller state to be sent to the plant for decryption and re-encryption at each time step, adding additional overhead. More recently, \cite{RTS_HME_FPGA} have demonstrated that it is possible to implement a direct feedback control scheme utilising the PHE scheme by \cite{Paillier}.
Due to the limited homomorphic properties of the scheme, the controller used un-ecnrypted controller gains, which might pose a security risk.

Furthermore, FHE schemes have also been proposed for control, such as by \cite{PeriodicReset,Kim2016,Quant_proj,Kim2021,Chaher2021}. %However, to the authors knowledge no implementation of FHE for control has been published.% **Any other example of HME applied for control** **Either a source where FHE is used for control or if there is none, mention that no implementation with FHE has been attempted**
All these FHE schemes however still suffer from two problems. Firstly, each scalar signal encrypted with FHE becomes a matrix cipher that need orders of magnitude more storage than the original signal. This means that real-time control with FHE requires large amounts of computation power, memory, and communication bandwidth. This limits the possible complexity of the controller and the minimum update rate. Such as in \cite{Kim2016}, where a two-state LTI controller with unencrypted control parameters is implemented with an update rate of $2~Hz$. Furthermore, in \cite{Cheon2018} a real-time implementation of a direct measurement feedback controller with FHE is presented for high-level control of a drone at an update rate of $10~Hz$.%  **Any methods attempting reduced computation complexity or using fast, dedicated, hardware?**

Secondly, PHE and FHE only allow for encryption of unsigned integers. Most control applications require the representation of fractional numbers as well as negative numbers. Unsigned integers can be made to represent positive and negative fractions using fractional bit representation. These numbers are commonly called fixed precision numbers.
% Secondly, FHE only allows for encrypting integers, whereas most control applications require the representation of fractional numbers, commonly represented as fixed precision numbers. 

% the implementation of which is not trivial when utilising HME. %Though some work on encrypting floating point number using HME \citep{FHE_Float} does exist, the required logic it considerably more complex. 
%A commonly used approach is to utilise fixed precision numbers to represent fractional. %When multiplying two fixed precision numbers, its precisio

When fixed precision numbers are multiplied, the decimal point of the result will shift by the amount of fractional digits of the two input values. Given limited precision, successive multiplications can shift the decimal point beyond available register size, causing overflow. The traditional solution to regain the original precision and prevent this overflow is to perform a right bit-shift on the multiplication result. Unfortunately, there is no known property of FHE which allows right bit-shifts on encrypted data.

% When fixed precision numbers are multiplied, their precision has to be increased to obtain an exact result. With a limited size in which the number is stored, this will at some point lead to overflow. The traditional solution to regain the original precision and prevent this overflow is performing a right bit-shift. The problem for FHE is that a method to perform a right bit-shift on encrypted data does not currently exist. 
%  to prevent overflow, which has not been possible yet.
%To prevent overflow when multiplying encrypted fixed precision numbers, solutions such as 
As alternative solutions, a periodic reset \citep{PeriodicReset} and scaling of the state space matrices \citep{Quant_proj} have been proposed to solve the problem of overflow. These methods however have implications for the stability of the controlled system, which limits the types of control to which they are applicable.
%The downside to such schemes is that they suffer from limited multiplicative depth (uitleg).

%ADVANTAGES (and difficulties) of HME specific to control
%Due to the way FHE operates, numbers are stored as large matrices. The communication and processing of these large amounts of data makes practical implementation of FHE a hard task. As such, no practical implementation has been presented that can perform real-time feedback control using FHE.

The problems of computational complexity and fixed precision limitations has meant application of FHE for real-time control has been limited. In this paper we will propose an FHE scheme for real-time safe control implemented on an FPGA. To this end we present the following contributions:
\begin{itemize}
    \item To mitigate the required hardware resources for FHE, a so-called \emph{reduced cipher} is introduced via a change of representation of the original cipher. Use of this reduced cipher for homomorphic operations significantly reduces their computational complexity.
    %\item A transformation of the (reduced) cipher is introduced with which it becomes possible to use FHE for control with fixed precision fractional numbers. 
    \item The FHE scheme is implemented on a Field Programmable Gate Array (FPGA) such that optimal use can be made of the novel \emph{reduced cipher}.
\end{itemize}
The resulting FHE scheme can be used in combination with any existing digital control scheme. The FHE scheme will be implemented for the control of an inverted double pendulum. It will be shown that the encrypted controller is able to run in real-time and stabilize the plant around an unstable equilibrium.

The remainder of the paper is structured as follows. In Section \ref{sec:prob} the considered control setup as well as the current problems with FHE in control will be introduced in more detail. In Section \ref{sec:fpga} the proposed solutions to these problems are introduced and proven. Section \ref{sec:results} then shows results obtained when implementing FHE on an FPGA for control of a inverted double pendulum. Lastly, the paper is concluded in Section \ref{sec:concl}.

%will present a practical implementation of FHE used for real-time secure feedback-control on a set of FPGA's.
%For a control system, it is required to represent fractions. HME schemes can only represent integer values and so fractional bit representation is utilised (ref). When two fractional bit numbers are multiplied, the amount of bits that represent the fractional portion of the grows. To counteract this issue, normally a right hand bit shift would be performed for truncation, wich is the equivalent of devision by a power of two. However, both PHE (paillier) and FHE allow for multiplication, but not division. In previous work, workarounds had to be found, such as performing a periodic reset (ref). This is to the detriment of the stability and smoothness of operation of the system. 

%In this paper we present a method to perform truncation of encrypted numbers. This allows for the implementation of conventional control systems. 

%In this paper we present a change of representation that allows for the efficient implementation of FHE Encryption and homomorphic operations. This change of interpretation allows for efficient implementation on FPGA's and also lends itself for more efficient implementation on hardware with fixed register sizes. Furthermore, we introduce a method of performing right hand bit shifts on encrypted numbers. With these findings we have constructed a proof of concept of a fully homomorphic feedback control system, utilising conventional control to stabilise an upright inverse double pendulum.

%**Paragraph about hardware platforms that can be suited for computationally intensive tasks**

%Contribution of this paper


%- Security/Privacy Issues in Control\\
%- How Encryption can overcome this\\
%- Why fully homomorphic encryption can provide full security/privacy.\\
%- Existing methods for fully homomorphic encryption and appications.\\
%- Difficulties with fully homomorphic encryption for control.\\
%- Contribution of this research.\\
%- Overview of the paper.\\
\subsection{Notation} \label{ssec:notation}
If a positive scalar $x$ is considered to be in binary representation, we denote the individual digits of $x$ as $x^{[i]}$ such that $x=\sum_{i=0}^\infty 2^ix^{[i]}$. Furthermore, for any $x\in\mathbb{N}$ we can define $(x)^\ell=\sum_{i=0}^{\ell-1} 2^ix^{[i]}$ which is equivalent to the $\ell$ least significant binary digits of $x$, i.e. discarding overflow.% (i.e. if $x \geq q$, indices exceeding $\ell$ are not included in the sum).
Then denote $[x]^\ell=[x^{[0]},\dots,x^{[\ell]}]$ as a vector in which the digits of $(x)^\ell$ are treated as separate elements.
Furthermore, let us define $g = [2^0,\dots, 2^{\ell-1}]^\top$ %such that $[x]^\ell g=(x)^l$. Lastly, 
and denote the set $\mathbb{Z}_q = \{0,\dots,q-1\}$, where $q \in \mathbb{N}$. Lastly, we denote bit-shifts of a number $x$ by $i$ bits as $x\ll i =2^ix$ and  $x\gg i =2^{-i}x$.

These concepts can be extended to a matrix of arbitrary size $X\in \mathbb{N}^{n_1 \times n_2}$, where $(X)^\ell$, $[X]^\ell$, and bitshifts are applied element-wise. Furthermore, define $G_{n} = I_{n} \otimes g$.% such that $[X]^\ell G_{n_2} = (X)^\ell$.

Furthermore, we will denote the encrypted version of a variable $x$ as $E(x)$.
